Realtime Multilevel Crowd Tracking using Reciprocal Velocity Obstacles

We present a novel, realtime algorithm to compute the trajectory of each pedestrian in moderately dense crowd scenes. Our formulation is based on an adaptive particle filtering scheme that uses a multi-agent motion model based on velocity-obstacles, and takes into account local interactions as well as physical and personal constraints of each pedestrian. Our method dynamically changes the number of particles allocated to each pedestrian based on different confidence metrics. Additionally, we use a new high-definition crowd video dataset, which is used to evaluate the performance of different pedestrian tracking algorithms. This dataset consists of videos of indoor and outdoor scenes, recorded at different locations with 30-80 pedestrians. We highlight the performance benefits of our algorithm over prior techniques using this dataset. In practice, our algorithm can compute trajectories of tens of pedestrians on a multi-core desktop CPU at interactive rates (27-30 frames per second). To the best of our knowledge, our approach is 4-5 times faster than prior methods, which provide similar accuracy.

==> 5-2.tex <==


\section{Results}

\begin{figure*}[thb]
	\centering
		\includegraphics[width=1\textwidth]{images/Graph.png}
		\label{fig:9}
		\caption{We compare AdaPT with different online trackers. The first graph represents the average fps achieved on our test machine. The second graph represents the tracking accuracy. (Algorithms - Online Boosting\cite{babenko2009visual}, KMS\cite{comaniciu2003kernel}, SMS\cite{collins2003mean}, ASLA\cite{jia2012visual}, Frag\cite{adam2006robust}, Kalman Filter\cite{weng2006video}. Datasets - seq\_hotel\cite{pellegrini2009you}, seq\_eth\cite{pellegrini2009you}, zara01\cite{lerner2007crowds}, zara02\cite{lerner2007crowds})}
\vspace*{-0.13in}
\end{figure*}
%\begin{figure*}[!htb]
	%\centering
		%\includegraphics[width=1\textwidth]{images/Graph2.png}
		%\caption{}
	%\label{fig:6}
%\end{figure*}

In this section, we highlight the performance of our algorithm on different benchmarks and compare the performance with these prior techniques - \textit{Online Boosting}\cite{babenko2009visual}, \textit{KMS}\cite{comaniciu2003kernel}, \textit{SMS}\cite{collins2003mean}, \textit{ASLA}\cite{jia2012visual}, \textit{Frag}\cite{adam2006robust}, \textit{Kalman Filter}\cite{weng2006video}.
We compare the accuracy (in terms of pedestrians tracked in the video sequence) and speed (in terms of frames per second) of our algorithm on the following 4 datasets - BIWI Walking Pedestrians dataset (\textit{seq\_hotel and seq\_eth})\cite{pellegrini2009you} and Crowds by example (\textit{zara01, zara02})\cite{lerner2007crowds}. WHAT ABOUT INRIA DATASET THAT YOU CITED IN FIGURE 2

We tested these algorithms on an Intel\textcopyright Haswell, Core\textregistered  i7-4771 Processor (4 Cores). 8MB Cache, 3.90 GHz and Intel\textcopyright HD Graphics 4600. AdaPT is implemented in C++, and some components use OpenMP and OpenCL for exploiting multiple cores. MENTION WHICH COMPUTATIONS ARE PERFORMED ON SEPARATE CORES.
\begin{table}[H]
\caption{Crowd Scenes used as Benchmarks. We highlight many attributes of these videos. HOW MANY PEDESTRIANS THEY HAVE, ADD A COLUMN FOR THAT}
    \begin{tabular}{|l|l|}
    \hline
    seq\_hotel & Illumination Variation, Occlusion                                        \\ \hline
    seq\_eth   & Background Clutters, Illumination Variation, Low Resolution \\ \hline
    zara01    & Background Clutters, Illumination Variation, Occlusion  \\ \hline
    zara02    & Background Clutters, Illumination Variation, Occlusion                   \\ \hline
    \end{tabular}
		
\end{table}

